QDD-MM: A Simple and Compact Open-Source Muscle Module with Quasi-Direct-Drive Motor for Tendon-driven Robots

Tendon-driven robots, which actuate like biological muscles by using motors to wind wires, offer advantages such as variable stiffness and redundant actuation. Despite these advantages, musculoskeletal structures inherently involve a large number of diverse muscles, making it desirable to compactly modularize each muscle unit and flexibly accommodate diverse muscle arrangements. While various small muscle modules have been proposed to date, existing designs tend to be complex, difficult to maintain, and suffer from low backdrivability and limited actuation speed due to their high gear ratios. In this work, we propose QDD-MM, a muscle module that leverages recent advances in quasi-direct-drive motors to achieve a simpler and more compact structure with higher backdrivability and faster actuation than previous modules. By utilizing quasi-direct-drive motors, the module eliminates the need for dedicated force-sensing mechanisms, significantly simplifying the overall design, while also supporting flexible wire routing in multiple directions, various module-to-module connections, and even the use of the module body itself as a structural component. QDD-MM integrates these capabilities into a reusable muscle module, and its design is openly available at https://github.com/haraduka/qddmm. We developed tendon-driven robots with one joint and either two or three muscles, as well as a partial musculoskeletal humanoid, using the proposed QDD-MM and verified their effectiveness. We expect that this muscle module will democratize tendon-driven robotics and further accelerate progress in the field.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% for not arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
%      ]{hyperref}
% \usepackage[dvipdfmx]{graphicx}
% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

\usepackage{url}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}

\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}

\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\tabref}[1]{{Table~\ref{#1}}}
\newcommand{\figref}[1]{{Fig.~\ref{#1}}}
\newcommand{\equref}[1]{{Eq.~(\ref{#1})}}
\newcommand{\algoref}[1]{{Alg.~\ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

